Better Agnostic Clustering Via Relaxed Tensor Norms

We develop a new family of convex relaxations for $k$-means clustering based on sum-of-squares norms, a relaxation of the injective tensor norm that is efficiently computable using the Sum-of-Squares algorithm. We give an algorithm based on this relaxation that recovers a faithful approximation to the true means in the given data whenever the low-degree moments of the points in each cluster have bounded sum-of-squares norms. We then prove a sharp upper bound on the sum-of-squares norms for moment tensors of any distribution that satisfies the \emph{Poincare inequality}. The Poincare inequality is a central inequality in probability theory, and a large class of distributions satisfy it including Gaussians, product distributions, strongly log-concave distributions, and any sum or uniformly continuous transformation of such distributions. As an immediate corollary, for any $\gamma > 0$, we obtain an efficient algorithm for learning the means of a mixture of $k$ arbitrary \Poincare distributions in $\mathbb{R}^d$ in time $d^{O(1/\gamma)}$ so long as the means have separation $\Omega(k^{\gamma})$. This in particular yields an algorithm for learning Gaussian mixtures with separation $\Omega(k^{\gamma})$, thus partially resolving an open problem of Regev and Vijayaraghavan \citet{regev2017learning}. Our algorithm works even in the outlier-robust setting where an $\epsilon$ fraction of arbitrary outliers are added to the data, as long as the fraction of outliers is smaller than the smallest cluster. We, therefore, obtain results in the strong agnostic setting where, in addition to not knowing the distribution family, the data itself may be arbitrarily corrupted.

==> content/OLD_prelims.tex <==
%!TEX root=../main.tex
\section{Preliminaries}
We write $\Norm{v}$ for the Euclidean norm $\sqrt{ \sum_{i = 1}^n v_i^2}$ of a vector $v \in \R^n$ and $\Norm{A}$ for the spectral norm: $\sup_{v: \Norm{v} \leq 1 }|\langle v, A v \rangle|$ of a matrix $A$. 

\subsection{Tensors and Polynomials}
For us, $d$-dimensional tensors on $\R^n$ are a collection of numbers indexed by $d$-tuples of indices from $[n].$ A $d$-dimensional tensor on $\R^n$ is naturally associated with a homegenous degree $d$ polynomial $\langle T, x^{\otimes d}\rangle.$ The (symmetric) injective tensor norm of a $d$ dimensional tensor $T$ is defined as $\Norm{T}_{inj} = \sup_{v: \Norm{v} = 1} \langle T, v^{\otimes d} \rangle.$

Given a set of points $S$ and a $\mu \in \R^n$, we define the \emph{centralized $d$-moment tensor} of $S$ around $\mu$ as $M_d(S,\mu) = \eqdef \frac{1}{|S|} \sum_{y \in S} (y-\mu)^{\otimes d}.$ Observe that $M_2(S,\mu)$ is the covariance matrix of $S$ assuming $\mu$ is the mean of uniform distribution on $S$.

\subsection{Pseudo-distributions}
Let $\cP_d(n)$ be the set of all polynomials of degree at most $d$ over $\R^n$ and let $\cP(n) = \cup_{d > 0} \cP_d(n).$ Write $\deg(p)$ for the total degree of $p$. A degree $d$ pseudo-distribution $D$ on $\R^n$ is a finitely supported function $\D:\R^n \rightarrow \R$ such that for every $p \in \cP_{d/2}$, the \emph{pseudo-expectation} $\pE_{\D}$ functional defined by $\pE_{\D}[p] \eqdef \sum_{x:\D(x) > 0} \D(x) \cdot p(x)$ satisfies: $\pE_{\D}[1] = 1$ and $\pE_{\D}p^2 \geq 0$ for every $p \in \cP_{d/2}(n).$ $\D$ is a degree $\infty$ pseudo-distribution iff it is a finitely supported probability distribution over $\R^n.$

The key property of pseudo-distributions is that while there's can be no efficient separation oracle (assuming $P \neq NP$) for the convex set of degree $d$ moment tensors of probability distributions, there's a $n^{O(d)}$ time weak separation oracle for the convex set of degree $d$ moment tensors of degree $d$ pseudo-distributions. 

\begin{theorem}[\cite{MR1846160-Lasserre01}, \cite{parrilo2000structured}, \cite{MR1618100-Nesterov98}, \cite{MR939596-Shor87}]
There's a $n^{O(d)}$ time weak separation oracle (in the sense of \cite{MR625550-Grotschel81}) for the following convex set:
\[
\left\{ \pE_{\D}[ (1,x_1, x_2, \ldots, x_n)^{\otimes d}] \mid \D \text{ is a degree $d$ pseudo-distribution over $\R^n$ } \right\}
\]
\end{theorem}

\textbf{Constraints:} A pseudo-distribution $\mu$ is said to \emph{satisfy} a constraint $q(x) = 0$ if for every $p$ of degree at most $d-deg(q)$, $\pE_{\mu}[pq] = 0.$ We say that a pseudo-distribution $\mu$ is supported over the unit sphere if it satisfies the constraint $\sum_{i} x_i^2-1 = 0.$

\textbf{Sum-of-Squares Norms: } Pseudo-distributions are naturally associated with a family of norms that admit efficient algorithms for optimization on their unit balls. These norms can be seen as natural relaxation of the injective tensor norms of tensors and their duals. We define these next.

For a tensor $T \in (\R^{n})^{\otimes d}$, we define the degree $d$ sum-of-squares norm, written as 
\[
\Norm{T}^4_{\sos_d} \eqdef \sup_{\mu: \text{ degree d pseudo-distribution over $\bbS^{n-1}$}} \pE_{\mu}\langle T, x^{\otimes 4} \rangle
\]
It's not hard to show that if $T$ is a $2$ dimensional tensor (i.e., a matrix) then the $\Norm{T}_{\sos_2} = \Norm{T}$, the spectral norm of the matrix $T$. In general, $\Norm{T}_{\sos_d} \geq \Norm{T}_{inj}.$

% \textbf{Dual Norms: } 
% It's not hard to verify that the dual norm of 

\begin{definition}[Degree 4 Deviation]
For a subset $S$ of points in $\R^n$ and a \emph{center} $\mu \in \R^n$, we define degree 4 deviation of $S$ as follows: 
\[ \sigma(S,\mu) =   \Norm{M_4(S,\mu)}_{inj}. \]
\end{definition}

\subsection{Basic Concentration Tools}

\begin{definition}[Orlicz Norms]
Let $\psi:\R \rightarrow \R$ be an increasing, convex function on $\R$. The Orlicz $\psi$-norm of a random variable $X$ is defined as the $\{\inf c > 0: \E [ \psi(X/c) ] \leq 1].$
\end{definition}

We will be interested in exponential Orlicz norms: for each $0 \leq \alpha < 1$, let 
\[
\psi_{\alpha}(x) = \begin{cases} e^{x^{\alpha}} -1 \text{ if } x > (1-\alpha) \\
							     (\frac{1}{(1-\alpha)})^{1-\alpha}  \cdot x \text{  otherwise. }
					\end{cases}
\]
For $\alpha \geq 1$, we let $\psi_{\alpha}$ be $e^{x^\alpha}-1$. Observe that $\psi_{\alpha}$ is increasing and convex everywhere.

The following tail bound immediately follows from an Orlicz norm bound:
\begin{lemma}[Tail Bound from Orlicz Norm]
Let $X$ be a non-negative random variable such that $\norm{X}_{\psi_{\alpha}} = K$. Then, for every $t \geq (1-\alpha) \cdot K$, $\Pr[ X \geq t] \leq (e^{(t/K)^{\alpha}}-1)^{-1}.$ \label{lem:tail-via-Orlicz}
\end{lemma}
\begin{proof}
By Markov's inequality, $\Pr[ X \geq t] \leq \Pr[ \psi(X/K) \geq \psi(t/K)] \leq \E[ \psi_{\alpha}(X/K)]/\psi_{\alpha}(t/K) \leq \psi_{\alpha}(t/K).$ The bound now follows by noting that for, $t \geq (1-\alpha)K$, $\psi(t/K) = e^{(t/K)^{\alpha}}-1.$

\end{proof}

Orlicz norms allow simple arguments for obtaining concentration inequalities involving sums of independent random variables. The following is the key tool in showing such results.

\begin{fact}[Ledoux-Talagrand, \cite{probabilityinbanachspaces}, Theorem 6.2]
There exists a constant $K_{\alpha}$ depending on $\alpha$such that for a sequence of independent mean zero random variables $X_1, X_2, \ldots, X_m$ with bounded $\psi_{\alpha}$ norms and $0 \leq \alpha \leq 1$, 
\begin{equation}
\Norm{\sum_{i = 1}^m X_i}_{\psi_{\alpha}}\leq K_{\alpha} \left(  \Norm{\sum_{i = 1}^m X_i}_1 + \Norm{\max_{i \leq m} \norm{X_i}}_{\psi_{\alpha}}  \right) \label{eq:conc-Ledoux-talagrand}
\end{equation} \label{fact:ledoux-talagrand}
\end{fact}

To bound the Orlicz norm appearing on the RHS of \eqref{eq:conc-Ledoux-talagrand}, the following result comes in handy:

\begin{fact}[] \label{fact:supremum-orlicz}

There exists an absolute constant $c > 0$ such that for any real valued random variables $X_1, X_2, \ldots, X_m$, 
\[
\Norm{ \max_{i \leq m} |X_i| }_{\psi_{\alpha}} \leq c \psi_{\alpha}^{-1}(m) \cdot \max_{i \leq m} \norm{X_i}_{\psi_{\alpha}}.
\]
\end{fact}

To estimate Orlicz norms of random variables under simple transformations, we will use the following simple-to-prove fact:

\begin{fact} \label{fact:Orlicz-of-product}
Let $X,Y$ be two (potentially correlated) random variables, with  $\psi_{\alpha}$ norm bounded by $a$ and $b$ respectively. Then, $\norm{XY}_{\psi_{\alpha/2}} \leq D_{\alpha} a b$ for some constant $D_{\alpha}$ depending only on $\alpha$. 
\end{fact}



Fact \ref{fact:supremum-orlicz} combined with Fact \ref{fact:ledoux-talagrand} immediately yields the following estimate for Orlicz norms of sums of independent random variables in terms of the Orlicz norms of the individual summands:

\begin{lemma}
For any $0 \leq \alpha \leq 1$, there exists a constant $K_{\alpha}$ such that for a sequence of independent random variables $X_1, X_2, \ldots, X_n$, 
\begin{equation}
\Norm{\sum_{i = 1}^m X_i - \E [ \sum_{i = 1}^m X_i]}_{\psi_{\alpha}} \leq K_{\alpha} \sqrt{m} \log{(m)} \max_{i \leq m} \norm{X_i}_{\psi_{\alpha}}.
\end{equation}
\end{lemma}

Using Lemma \ref{lem:tail-via-Orlicz}, we thus obtain the following tail bound as the corollary.


\begin{corollary}[Concrete Tail Bound] \label{cor:concrete-tail-bound}
Let $X_1, X_2, \ldots,X_m$ be a sequence of independent non-negative real valued random variables. Let $t_0 = K_{\alpha} \sqrt{m} \log(m) \max_{i \leq m} \norm{x_i}_{\psi_{\alpha}}$. Then, for any $t \geq t_0/m$,
\[
\Pr[ \frac{1}{m}\sum_{i = 1}^m X_i - \frac{1}{m}\E[ \sum_{i = 1}^n X_i] > t]\leq 
(e^{(mt/t_0)^{\alpha}}-1)^{-1}.
\]
\end{corollary}


==> content/applications.tex <==
\section{Application: Mixtures of Poincar\'e Distributions}
\label{sec:applications}

In this section we give corollaries of our results for learning mixtures of 
Poincar\'e distributions, and in particular mixtures of Gaussians. Given a 
mixture of $k$ distributions with corresponding means $\mu_1, \ldots, \mu_k$, 
we define the separation $\Delta = \min_{j \neq j'} \|\mu_j - \mu_{j'}\|_2$, 
which affects the difficulty of clustering.

A simple corollary of our results is the following:

\begin{corollary}[Disentangling Mixtures of Arbitrary \Poincare Distributions]
\label{cor:poincare-mixture}
Suppose that we are given a dataset of $n$ points $x_1, \ldots, x_n$, 
such that at least $(1-\epsilon)n$ points are drawn from a mixture 
$\alpha_1p_1 + \cdots + \alpha_kp_k$ of $k$ distributions, where 
$p_j$ is $\sigma$-Poincar\'e around $\mu_j$ (the remaining $\epsilon n$ 
points may be arbitrary). Let $\alpha = \min_{j=1}^k \alpha_j$. 
Also suppose that the separation $\Delta$ is at least 
$\Csep \cdot C_t \sigma / \alpha^{1/t}$, for some universal constant $C_t$ 
and some $\Csep \geq 1$.

Then, assuming that $\epsilon \leq \frac{\alpha}{10}$, 
for some $n = \oo((2d\log(tkd/\delta))^t/\alpha + d\log(k/\delta)/\alpha\epsilon^2)$, 
there is an algorithm running in $n^{\oo(t)}$ time which with probability 
$1-\delta$ outputs 
candidate means $\hat{\mu}_1, \ldots, \hat{\mu}_k$ such that 
$\|\hat{\mu}_j - \mu_j\|_2 \leq C_t' \sigma (\epsilon / \alpha + \Csep^{-2t})^{\frac{2t-1}{2t}}$ 
for all $j$.
\end{corollary}
This is a direct consequence of Theorem~\ref{thm:cert} 
and Theorem~\ref{thm:clustering-separated}, where the extra term of 
$d\log(k/\delta)/\alpha\epsilon^2$ in the sample complexity is necessary for the 
empirical means of each cluster to concentrate to the true means.

Note the $\Csep^{-2t}$ term---this says that as the clusters become increasingly well-separated, 
it is possible to estimate the means with smaller and smaller error. However, 
even if the fraction of outliers $\epsilon \to 0$, the error is non-vanishing for any 
finite amount of separation. This is information-theoretically necessary because 
two clusters could overlap slightly in the tails, and it is in general not possible to tell 
which of the two clusters a point in the overlap should belong to.

In the case of mixtures of Gaussians, however, we can in fact get vanishing error:
\begin{corollary}
\label{cor:gaussian-mixture}
Suppose that $x_1, \ldots, x_n \in \bR^d$ are drawn from a mixture of 
$k$ Gaussians: $p = \sum_{j=1}^k \alpha_j \sN(\mu_j, I)$, where 
$\alpha_j \geq 1/\poly(k)$ for all $j$. 
Then for any $\gamma> 0$, there is a separation $\Delta_0 = \oo(k^{\gamma})$ 
such that given $n \geq \poly(d^{1/\gamma}, k, 1/\epsilon)\log(k/\delta)$ samples from  
$p$, if the separation $\Delta \geq \Delta_0$, then with probability $1-\delta$ 
we obtain estimates 
$\hat{\mu}_1, \ldots, \hat{\mu}_k$ with $\|\hat{\mu}_j - \mu_j\|_2 \leq \epsilon$.
\end{corollary}
Note that now the error actually goes to $0$ as $n \to \infty$, which is 
not true in Corollary~\ref{cor:poincare-mixture}. This is by invoking 
Theorem IV.1 of \citet{regev2017learning}, which says that any sufficiently good 
initial estimates of a mixture of Gaussians can be amplified to get arbitrarily good accuracy.
Note that such a result is specific to Gaussians and, as noted above,
is information-theoretically impossible for mixtures of general Poincar\'e distributions.

Corollary~\ref{cor:gaussian-mixture} is a direct consequence of 
Corollary~\ref{cor:poincare-mixture} (used to make the error in the initial estimates 
$\hat{\mu}_j$ small enough) together with \cite{regev2017learning}'s 
amplification result.


==> content/proof.tex <==
%!TEX root=../main.tex
\section{The Problem}
In this section, we formulate the clustering problem under the well-separated centers assumption. We will refer to this as the clusterning problem from here on.

\noindent \textbf{Input:} $m$ points $x_1, x_2, \ldots, x_m \in \R^n.$


\noindent \textbf{Promise: } There exist a partition of $[m]$ into disjoint sets $S_1, S_2, \ldots, S_k$, cluster means $\mu_1, \mu_2, \ldots, \mu_k \in \R^n$ and cluster deviation bounds $0 \leq \sigma_2,\sigma_4$ such that
\begin{enumerate} 
\item \textbf{Bounded Norm: } $\Norm{\mu_i} \leq r$ for some parameter $r$, \Pnote{This is perhaps not needed.}
\item \textbf{Well-Separated Centers: } There exists a $C > 0$ such that $\Norm{ \mu_i - \mu_j} \geq C k^{\frac{1}{4}} \sigma$ whenever $i \neq j$ and, 
\item \textbf{2nd moment bound on clusters: } For $1 \leq j \leq k$, $\Norm{\frac{1}{|S_j|}\sum_{i \in S_j} \dyad{(x_i-\mu_j)}} \leq \sigma_2.$
\item \textbf{4th moment bound on clusters: } For $1 \leq j \leq k$, $\sup_{v: \norm{v} \leq 1} \frac{1}{|S_j|}\sum_{i \in S_j} \langle x_i-\mu_j, v \rangle^4 \leq \sigma_4^4.$
\end{enumerate}
\noindent \textbf{Goal: } Recover $\hat{\mu}_1,\hat{\mu}_2, \ldots, \hat{\mu}_k$ such that: $\Norm{\mu_i - \hat{\mu}_i} \leq .$

\section{The "Ideal" Relaxation}
The goal of this section is to present a natural polynomial feasibility formulation obtained by directly translating the conditions described in the problem formulation above. We will relax this formluation and obtain the convex program we use in the following section. 

\noindent \textbf{Variables: }
\begin{enumerate}
\item \textbf{ Cluster assignment variables: } $w_{i,j}$: $1 \leq i \leq m$, $1 \leq j \leq k+1$.
\item \textbf{ Cluster Centers: } $\mu_1, \mu_2, \ldots, \mu_k \in \R^n.$
\end{enumerate}

\noindent \textbf{Parameters: }
Deviation bound $\sigma$, norm bound $r$ and accuracy parameter $\delta \ll 1/k$.

\noindent \textbf{Constraints: }
\begin{align}
w_{i,j} &\geq 0 \notag \\
\norm{\mu_j} &\leq r \text{ } \forall 1 \leq j \leq k. \notag \\
\sum_{j} w_{i,j} &= 1 \notag \\
\sum_{i} w_{i,k+1} &\leq \delta m \notag  \\
\sup_{v: \norm{v} \leq 1} \sum_{i = 1}^m w_{i,j} \langle x_i - \mu_j, v \rangle^4 &\leq  \sum_{i} w_{i,j} \sigma_4^4 \text{ } \forall 1 \leq j \leq k. \notag \\ 
\sup_{v: \norm{v} \leq 1 } \sum_{i = 1}^m w_{i,j} \langle x_i - \mu_j, v \rangle^2 &\leq \sum_{i} w_{i,j} \sigma_2^2 \text{ } \forall 1 \leq j \leq k. \label{eq:polynomial-formulation}
\end{align} 

The program \eqref{eq:polynomial-formulation} is clearly non-convex and as such there's no reason to expect that one can find a solution (if one exists) to it efficiently. The main goal of this section is to establish that under the 2nd and 4th moment well-separated-centers conditions, any solution to the above program recovers cluster centers that are close to the true cluster centers $\mu_i$s. Obtaining a convex relaxation of the above program and arguing that solutions to it can be rounded to a get good cluster centers is the objective of the next section. 

\section{Certifying Injective Norms of 4th Moment Tensors}
In the convex optimization program that we develop for clustering, we are interesting in finding $\mu$ such that $\Norm{M_4(S,\mu)}_{inj} \leq \tau$ for parameters $S$ and $\tau$. However, the unit ball of injective tensor norm doesn't admit an efficient separation oracle and thus such a constraint makes the program hard to solve efficiently. Our idea here is  to instead force a constraint in terms of some efficiently computable relaxation of the injective norm - the natural choice being the sum-of-squares norm of degree 4 of $M_4(S,\mu).$ However, $\Norm{M_4(S,\mu)}_{\sos_4} \geq \Norm{M_4(S,\mu)}_{inj}$ and thus, the constraint we are forcing is in general stronger than the one we are guaranteed to be feasible. 

If the $\sos_4$ norm and the injective norms of $M_4$ were within a constant factor of each other - then we'd get away with some additional constant factor in the error in recovering the centers which translates into a slightly larger constant factor in the separation conditions on the cluster means. However, if the gap between the two norms is dimension dependent, such a strategy fails miserably. Thus, we want to understand how far can the $\sos_4$ norm and the injective tensor norm of $M_4(S,\mu)$ be. 

It turns out that we are quite a bit out of luck here. Injective tensor norm for general tensors is known to be hard and there's no known algorithm that obtains an approximation factor of $o(n)$ for 4-dimensional tensors. While one may expect the situation for moment tensors to be different, unfortunately, there's no better algorithm known even for this special case. Further, the problem of computing injective norm of the 4th moment tensor is studied as the well-known 2 to 4 norm problem classical approximation algorithm design and quantum information theory and is known to be harder than the notorious small set expansion problem (a variant of the unique games problem). Known hardness results already rule out constnat factor approximation algorithm for the problem in polynomial time \cite{DBLP:journals/jacm/HarrowM13}. The bottom line is that we  expect the degree 4 sum-of-squares norm to be some fixed polynomial factor in the dimension off from injective tensor norm of the 4th moment tensor around $\mu.$ 

A priori, this appears like a challenging obstable to overcome. Our main contribution here is to show that the degree 4 sum-of-squares algorithm (which computes the degree 4 sum-of-squares norm) on the 4th moment tensor around $\mu$ of $S$ achieves a constant factor approximation in a sense that is useful to us in our clustering setting but (as is inherently forced) doesn't provide a new approximation algorithm in the standard sense. This is the goal of the present section. 

Our sharper bounds on clustering would need a mild regularity assumption namely, that each cluster is made up of i.i.d. points from distribution with that allows concentration of convex Lipschitz functions (but with arbitrary dependency between the coordinates of the vectors). We precisely define this property below:

\begin{definition}[Convex Concentration Property] A random vector $x \in \R^n$ is said to have the convex concentration property with constant $K$ if for every $1$-Lipschitz convex function $\phi:\R^n \rightarrow \R$, $\E[\phi(x)] < \infty$ and for every $t > 0$, 
\[
\Pr[ |\phi(x) - \E[\phi(x)| \geq t] \leq 2 \exp(t^2/K^2).
\]
\end{definition}

 We will show that for any random vector satisfying the convex concentration property, a natural sum-of-squares relaxation gives a good approximation for the 2 to 4 norm. This extends the known results on SoS certificates for 2 to 4 norm for random operators  - the best known result in this regime is due to \cite{DBLP:conf/stoc/BarakBHKSZ12} who showed a similar result for i.i.d points from a distribution where each coordinate is an independent sub-gaussian scalar random variable. Key ingredient in the proof here is a sharp concentration bound for polynomials of random vectors that satisfy the concentration property mentioned above. 



% We then move on to the more general setting. Here, as discussed above, approximation in the standard sense cannot be expected. Instead, we show that for every collection of points $S$, there's a sub-collection of $0.9$ fraction of the points such that degree sum-of-squares norm and the injective norm of the 4th moment tensor of the sub-collection around $\mu$ are within a constant factor of each other.  As we show in the next section, this is enough for our purposes.



% We start with the definition of sub-gaussian distributions:

% \begin{definition}[Sub-Gaussian Random Vectors]
% A random variable $x \in \R^n$ is said to be sub-gaussian, if there exists a $\sigma > 0$ such that for every $\alpha \in \R^n$, $\E[ \exp( \alpha^{\top} x ) ] \leq \exp ( \norm{\alpha}^2 \sigma^2/2).$ We define the sub-gaussian norm of $x$ to be $\Norm{x}_{\psi_2} = \sup_{\alpha \in \bbS^{n-1}} \sqrt{2\log{\E[ \exp( \alpha^{\top} x ) ]}}$ if it exists.
% \end{definition}

% Observe that coordinates of a sub-gaussian random vector $x$ need not be independent. %Natural examples include standard spherical gaussian distribution (where the $\psi_2$ norm is $1$). 

The following tail estimate for polynomials of random vectors with convex concentration property will be useful to us:
% \Pnote{we need a different version unfortunately so might have to prove it ourselves - the Hsu-Kakade-Zhang result doesn't argue that polynomials concentrate around their means, I think that should be important to us since $\sigma^2 \tr(P)$ seems too large of an estimate for the mean.}

\begin{fact}[Adamczak ]
Let $x$ be a mean zero random variable in $\R^n$ that satisfies the convex concentration property with constant $\sigma$. Let $P$ be any $n \times n$ matrix. Then, there exists an absolute constant $C>0$ such that for every $t > 0$,
\begin{multline}
\Pr[ |\langle x, Px \rangle - \E[\langle x, Px\rangle]| \geq t] \leq 2 \exp\left(-\frac{1}{C\sigma^2} \cdot \min\{ \frac{t^2}{\norm{P}_F \cdot \norm{Cov(P)}}, \frac{t}{\norm{P}}\}\right)\\ \leq 2 \exp\left( -\frac{1}{C}\min\{\frac{t^2}{2\sigma^4\norm{P}_F^2},\frac{t}{\sigma^2\norm{P}}\}\right).
\end{multline}
\end{fact}
% We will need the following slightly refined version for our purposes - we prove this version in the appendix. 

% \begin{lemma}[Upper Tail Inequality for Polynomials of Sub-gaussian] \label{lem:upper-tail-subgaussian}
% Let $x$ be a mean zero, sub-gaussian random variable with $\psi_2$ norm $\sigma$ and covariance $\Sigma$. Let $P \succeq 0$ be any positive semidefinite matrix. Then, for every $t > 0$,
% \[
% \Pr\left[ \langle x, Px \rangle - \tr(\Sigma \cdot P) \geq  \sigma^2 \cdot \left(2 \sqrt{\tr(P^2)t} + 2 \norm{P}t\right)\right] \leq e^{-t}.
% \]
% \end{lemma}

The lemma along with Fact \ref{fact:Orlicz-of-product}  immediately implies a $\psi_{1/2}$ norm bound for the random variable $\langle x, Px \rangle$ for any $P \succeq 0$, $\norm{P}_F = 1.$

\begin{lemma} \label{lem:orlicz-polynomial}
Let $P \in \R^{n \times n}$ satisfy $\norm{P}_F = 1$. Let $x$ be a mean zero random variable that satisfies the convex concentration property with constant $\sigma$ and covariance $\Sigma.$ Then, $\norm{\langle x, P x\rangle - \tr(\Sigma \cdot P)}_{\psi_{1/2}} \leq  O(\sigma^2).$
\end{lemma}

We are now ready to show the main result of this section.
% namely that the matrix $\E[ x^{\otimes 2} x^{\otimes 2}^{\top}] \preceq \Theta(1) \cdot ( \Sigma \Sigma^{\top} + \sigma^4 \Id).$ 

\begin{theorem}[Majorization of 4th Moment Tensor]
Let $x_1, x_2, \ldots, x_m$ be i.i.d. from distribution satisfying the convex concentration property with constnat $\sigma >1$ and covariance $\Sigma$ for $m \geq n^8$\Pnote{this looks ginormous right now, but perhaps can be improved}. Then, with probability at least $1-e^{-\Omega(n^2)}$, there exists an absolute constant $C> 0$ such that $C\sigma^4 \Id - \frac{1}{m} \sum_{i = 1}^m \dyad{(x_i^{\otimes 2} -\Sigma)} \succeq 0.$
\end{theorem}

\begin{proof}
Let $M = \frac{1}{m} \sum_{i = 1}^m \dyad{(x_i^{\otimes 2}-\Sigma)}.$

We will argue that $C \sigma^4\Id-M \succeq 0$ for some large enough constant $C$. Let $\cB_{n^2} = \{P \in \R{n \times n} \mid \norm{P}_F = 1\}$ be unit sphere in $n^2$ dimension and let $\cN \subseteq \cB_{n^2}$ be a net with fineness $1/2.$ Then, $|\cN| \leq 2^{O(n^2)}.$

We will show that for some $C' > 0$, $\langle P^{\top}, MP \rangle \leq C'\sigma^4$ for every $P \in \cN.$ This implies that for $C = 2C'$, the same statement holds for every $P \in \cB_{n^2}$ and completes the proof for $C= 2C'.$

We now focus on showing that $\langle P^{\top}, MP \rangle \leq C' \sigma^4.$ Towards this, we will fix a $P$ and argue that the probability of $\langle P^{\top}, MP \rangle > C'\sigma^4$ is at most $2^{-\Theta(n^2)}$. A union bound will then complete the proof.

From Lemma \ref{lem:orlicz-polynomial} for $x$ distributed as $x_i$s, $\norm{\langle P^{\top}, (x^{\otimes 2}-\Sigma) \rangle  }_{\psi_{1/2}} \leq K\sigma^2$ for some constant $K$. 

Using Fact \ref{fact:Orlicz-of-product}, there exists a constant $K' > 0$ such that
\[
\norm{\langle P, (x^{\otimes 2}-\Sigma) \rangle^2}_{\psi_{1/4}} \leq K'\sigma^4.
\]

% Thus, $\norm{\langle P^{\top}, x^{\otimes 2} \rangle^2}_{\psi_{1/4}} \leq K'' (\sigma^4 + \tr(\Sigma \cdot P)^2)$ for some constant $K''.$ 

We now apply Corollary \ref{cor:concrete-tail-bound} to the random variable $\langle P, (x^{\otimes 2}-\Sigma) \rangle^2$ and conclude that

% Applying Lemma \ref{cor:concrete-tail-bound} to $\langle P^{\top}, M P \rangle - \tr(\Sigma \cdot P) = \frac{1}{m} \sum_{i = 1}^m \langle P, x_i^{\otimes 2}} \rangle - \tr(\Sigma \cdot P))$ and using $t_0 = \Theta( \sqrt{m} \log{(m)} K\sigma^4)$ yields:

\[
\Pr[ |\langle P^{\top}, M P \rangle| \geq tC'\sigma^4)] \leq (e^{(mtK''\sigma^4/t_0)^{1/2}}-1)^{-1}.
\]

For $m =  \Omega(n^{8} \log{(n)})$, the RHS of the above is at most $2^{-\Theta(n^2)} \ll \frac{1}{|\cN|}$ as required.


% We are going to show that with probability at least $1-e^{-n}$ for every $A \in \R^{n \times n}$ such that $\norm{A}_F = 1$, the quadratic form $\langle A, M A \rangle \leq \langle Q, M Q \rangle.$ First, WLOG, we can assume that $A$ is Hermitian since $M$ shares the same symmetries. Next, we argue that it's enough to upper bound the quadratic forms of all $A \succeq 0$ with $\norm{A}_F = 1$. To see this, we write any matrix $A$ with $\norm{A}_F = 1$ as $A_1 - A_2$ for an orthogonal pair of psd matrices $A_1, A_2$ satisfying $\norm{A_1}_F, \norm{A_2}_F \leq 1.$

% By Cauchy-Schwarz inequality, we must have:
% $\langle A, M A \rangle \leq 2(\langle A_1, M A_1 \rangle + \langle A_2 , M A_2 \rangle).$



\end{proof}


==> content/robust-mean.tex <==
\section{Robust Mean Estimation via $2 \to q$-norm}

\Jcomment{this section is mostly complete but not sure how smooth the exposition is; also a few places where lemmas don't quite line up with how they're invoked, and some minor results that should be pushed to appendix}

\Jcomment{probably also good to be clear (here or in intro) what in this section is basically in 
\citet{steinhardt2017resilience} and what is new}

\Jcomment{TODO: possibly include stuff on covariance estimation if we figure it out}

This section will be dedicated to the following result:

\begin{theorem}
Suppose that $p$ is a distribution satisfying the Poincare inequality with 
parameter $\sigma$. Then, for any even $m \geq 2$, if we observe $n = \Omega(d^{m/2})$ 
samples from $p$, with an $\epsilon$ fraction of corruptions, it is possible to 
estimate the mean $\mu = \bE_p[x]$ to error 
$\|\hat{\mu} - \mu\|_2 = \oo(\epsilon^{1-1/m}\sigma)$.
\end{theorem}

The algorithm is based on the following optimization problem. Let 
$\sP_m$ be the family of degree-$m$ pseudodistributions over the unit sphere, 
so that $\max_{Y \in \sP_m} (\langle Y, \sum_{i=1}^n a_i^{\otimes m} \rangle)^{1/m}$ 
is a relaxation of the $2\to m$ norm of the matrix $A = [a_1 \ \cdots \ a_n]$.
We will let $\sW(\epsilon)$ denote the set of matrices $W \in \bR^{n \times n}$ satisfying 
$0 \leq W_{ij} \leq \frac{1}{(1-\epsilon)n}$ and $\sum_j W_{ij} = 1$ for all $i$.
The optimization problem is
\begin{equation}
\min_{W \in \sW(5\epsilon/3)} \max_{Y \in \sP_m} \frac{1}{n} \sum_{i=1}^n c_i \langle Y, (x_i - Xw_i)^{\otimes m} \rangle,
\end{equation}
where the $c_i$ are weights that start out at $1$ and are updated to downweight likely outliers.
The full algorithm is given as Algorithm~\ref{alg:robust-mean}.

\begin{algorithm}[b!]
\caption{Algorithm for robustly recovering the mean.}
\label{alg:robust-mean}
\begin{algorithmic}[1]
\STATE Initialize $c_i = 1$ for all $i=1,\ldots,n$ and $\sA = \{1,\ldots,n\}$.
  \STATE Let $Y \in \sP_m$ and $W \in \bR^{\sA \times \sA}$ 
  be the maximizer/minimizer of the saddle point problem
\protect\label{line:begin-loop}
%  \vskip -0.04in
  \begin{equation}
  \label{eq:opt-2}
  \max_{Y \in \sP_m} \min_{W \in \sW(5\epsilon/3)} \sum_{i \in \sA} c_i \langle Y, (x_i - X_{\sA}w_i)^{\otimes m} \rangle.
  \end{equation}
%  \vskip -0.10in \phantom{x}
  \IF{$\sum_{i \in \sA} c_i(x_i - X_{\sA}w_i)^{\top}Y(x_i - X_{\sA}w_i) > 4n\sigma^m$} 
\protect\label{line:if}
    \STATE Let $\tau_i = (x_i - X_{\sA}w_i)^{\top}Y(x_i - X_{\sA}w_i)$.
    \STATE For $i \in \sA$, replace $c_i$ with $\p{1-\frac{\tau_i}{\tau_{\max}}}c_i$, where $\tau_{\max} = \max_{i \in \sA} \tau_i$.
\label{line:outlier-begin}
    \STATE For all $i$ with $c_i < \frac{1}{2}$, remove $i$ from $\sA$.
\label{line:outlier-end}
    \STATE Go back to line \ref{line:begin-loop}.
  \ENDIF 
\protect\label{line:endif}
\STATE Output the average of the columns of $X_{\sA}$.
\end{algorithmic}
\end{algorithm}

\begin{proposition}
Suppose that $\epsilon \leq 0.075$, and that there is a set $S$ of 
$(1-\epsilon)n$ of the $x_i$ with empirical mean $\mu$ satisfying 
$\langle Y, \frac{1}{|S|} \sum_{i \in S} (x_i - \mu)^{\otimes m} \rangle \leq \sigma^m$ 
for all $Y \in \sP_m$. Then, the output $\hat{\mu}$ of Algorithm~\ref{alg:robust-mean} 
satisfies $\|\hat{\mu} - \mu\|_2 = \oo(\sigma \epsilon^{1-1/m})$.
\end{proposition}

\begin{proof}
We first make use of a lemma from \cite{steinhardt2017resilience} which analyzes 
lines \ref{line:outlier-begin}-\ref{line:outlier-end} of Algorithm~\ref{alg:robust-mean}; 
we reproduced it here:
\begin{lemma}
\label{lem:outlier}
For any scalars $\tau_i$ and $a$, suppose that $\sum_{i \in \sA} c_i\tau_i \geq 4a$ while 
$\sum_{i \in S \cap \sA} c_i\tau_i \leq (1-\epsilon)a$. Then the following 
invariants are preserved by lines \ref{line:outlier-begin}-\ref{line:outlier-end} of 
Algorithm~\ref{alg:robust-mean}: (i) $\sum_{i \in S} (1-c_i) \leq \frac{1-\epsilon}{4} \sum_{i=1}^n (1-c_i)$, and (ii) $|S \cap \sA| \geq (1-5\epsilon/3)n$.
\end{lemma}
Now, by Lemma~\ref{lem:outlier}, we know that when we reach 
line \ref{line:endif} of Algorithm~\ref{alg:robust-mean}, we have a set of points such that 
$\sum_{i \in \sA} c_i \langle Y, (x_i - X_{\sA}w_i)^{\otimes m} \rangle \leq 4n \sigma^m$ for 
all $Y \in \sP_m$. Moreover, $|\sA| \geq (1-5\epsilon/3)n \geq \frac{7}{8}n$, and $c_i \geq \frac{1}{2}$, and the set $\sP_m$ is a relaxation of $\{v^{\otimes m} \mid \|v\|_2 \leq 1\}$. Therefore, we also have
\begin{equation}
\frac{1}{|\sA|} \sum_{i \in \sA} \langle x_i - X_{\sA}w_i, v \rangle^m \leq \frac{64}{7} \sigma^m \|v\|_2^m \leq 10 \sigma^m \|v\|_2^m.
\end{equation}
In terms of the $2 \to m$ norm, we can re-interpret this as 
$\|(X_{\sA} - X_{\sA}W)^{\top}\|_{2 \to m} \leq 10^{1/m} \sigma$.

Let $u$ be the average of the columns of $W$, so that $u$ and $\Ind^{\top}$ are the top 
left and right singular vectors of $W$. We will show that the columns of $X_{\sA}$ have bounded 
moments around the point $X_{\sA}u$; this is equivalent to bounding 
$\|(X_{\sA} - X_{\sA}u\Ind^{\top})^{\top}\|_{2 \to m} = \|X_{\sA} - X_{\sA}u\Ind^{\top}\|_{\frac{m}{m-1} \to 2}$. We can do this as follows:
\begin{align}
\|X_{\sA} - X_{\sA}u\Ind^{\top}\|_{\frac{m}{m-1} \to 2} 
 &= \|(X_{\sA} - X_{\sA}W)(I - (W - u \Ind^{\top}))^{-1}\|_{\frac{m}{m-1} \to 2} \\
 &\leq \|X_{\sA} - X_{\sA}W\|_{\frac{m}{m-1} \to 2} \|(I - (W - u \Ind^{\top}))^{-1}\|_{\frac{m}{m-1} \to \frac{m}{m-1}} \\
 &\leq 10^{1/m} \sigma \|(I - (W - u \Ind^{\top}))^{-1}\|_{\frac{m}{m-1} \to \frac{m}{m-1}}.
\end{align}
By Corollary~\ref{cor:m-to-m-inv}, since $W \in \sW(5\epsilon/3)$ and $5\epsilon/3 \leq \frac{1}{8}$, we have $\|(I - (W - u \Ind^{\top}))^{-1}\|_{\frac{m}{m-1} \to \frac{m}{m-1}} \leq \frac{7}{3}$, so we have 
$\|X_{\sA} - X_{\sA}u\Ind^{\top}\|_{2 \to m} \leq \frac{7}{3} 10^{1/m} \sigma \leq 7.5\sigma$ (for $m \geq 2$).

To finish, we will consider the set $\sA \cap S$, and show that its mean is close to both 
the mean of $S$ and the mean of $\sA$. 
%This follows the same argument as in 
%\cite{steinhardt2017resilience} (in the language of that paper, it is a consequence of 
%resilience of the sets $\sA$ and $S$). 
Essentially, if any set $\tilde{S}$ has 
$m$th moments bounded by $\tilde{\sigma}$, then the mean of any set of $\epsilon |T|$ 
points in $T$ must differ from the mean of $T$ by at most $\tilde{\sigma} \epsilon^{-1/m}$ 
(as otherwise those points alone would cause the $m$th moments to exceed $\tilde{\sigma}$). 
Therefore, the mean of any set of $(1-\epsilon)|T|$ points differs from the overall 
mean by at most $\frac{\epsilon^{1-1/m}}{1-\epsilon}\tilde{\sigma}$. Applying this to both 
$S$ and $\sA$ with $\tilde{\sigma} = \sigma$ (for $S$) and $\tilde{\sigma} = 7.5\sigma$ 
(for $\sA$), and with $\epsilon = 5\epsilon/3$, we get that the means of $S$ and $\sA$ 
differ by at most 
$\frac{(5\epsilon/3)^{1-1/m}}{1-5\epsilon/3} \cdot 8.5\sigma \leq 16.2\sigma \epsilon^{1-1/m}$ 
(for $\epsilon \leq 0.075$), which completes the proof.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:outlier}]
We will show that if (i) and (ii) hold prior to the update in lines 
\ref{line:outlier-begin}-\ref{line:outlier-end}, then they will continue to hold.

Note that the amount that $\sum_{i \in S} c_i$ decreases in 
line \ref{line:outlier-begin} is proportional to $\sum_{i \in S \cap \sA} c_i\tau_i \leq (1-\epsilon)a$, while the amount that $\sum_{i=1}^n c_i$ decreases is proportional to 
to $\sum_{i \in \sA} c_i \tau_i \geq 4a$. Therefore, the former decreases at most 
$\frac{1-\epsilon}{4}$ times as fast as the latter, meaning that the invariant (i) 
is preserved.

Re-writing (i), we get $\sum_{i \in S} (1-c_i) \leq \frac{1-\epsilon}{4} \big(\sum_{i \in S} (1-c_i) + \sum_{i \not\in S} (1-c_i)\big)$. Re-arranging yields
$\sum_{i \in S} (1-c_i) \leq \frac{(1-\epsilon)/4}{1-(1-\epsilon)/4} \sum_{i \not\in S} (1-c_i) \leq \frac{1-\epsilon}{3+\epsilon} |[n] \backslash S| \leq \frac{\epsilon(1-\epsilon)}{3+\epsilon}n \leq \frac{\epsilon}{3}n$. In particular, $\{\#i \in S \mid c_i \leq \frac{1}{2}\} \leq \frac{2\epsilon}{3}n$, so at most $\frac{2\epsilon}{3}$ elements of $S$ are removed from $\sA$ in total. 
Therefore, $|S \cap \sA| \geq (1-5\epsilon/3)n$, so the invariant (ii) is preserved as well.
\end{proof}

\begin{lemma}
Suppose that $W \in \sW(\epsilon)$ and let $u$ be the mean of the columns of 
$W$. Then, for all $p \in [1,\infty]$, we have 
$\|W - u \Ind^{\top}\|_{p \to p} \leq \frac{(2\epsilon)^{1/p}}{1-\epsilon}$.
\end{lemma}
\begin{proof}
We have $\|W - u \Ind^{\top}\|_{p \to p} = \|W^{\top} - \Ind u^{\top}\|_{q \to q}$, where 
$q = \frac{p}{p-1}$. Furthermore,
\begin{align}
\|W^{\top} - \Ind u^{\top}\|_{q \to q} 
 &= \max_{\|v\|_q \leq 1} \big(\sum_{j=1}^n |\langle w_i - u , v \rangle|^q\big)^{1/q} \\
 &\stackrel{(i)}{\leq} \max_{\|v\|_q \leq 1} \big(\sum_{j=1}^n \|w_i - u\|_p^q \|v\|_q^q\big)^{1/q} \\
 &= \big(\sum_{j=1}^n \|w_i - u\|_p^q\big)^{1/q} \\
 &\stackrel{(ii)}{\leq} \big(\sum_{j=1}^n (\frac{(2\epsilon)^{1/p}}{1-\epsilon} n^{-1/q})^q\big)^{1/q} = \frac{(2\epsilon)^{1/p}}{1-\epsilon}.
\end{align}
Here (i) is H\"{o}lder's inequality while (ii) is the fact that
\begin{align}
\|w_i - u\|_p 
 &\leq \|w_i - u\|_1^{1/p} \|w_i - u\|_{\infty}^{1-1/p} \\
 &\leq (\frac{2\epsilon}{1-\epsilon})^{1/p} (\frac{1}{(1-\epsilon)n})^{1-1/p} \\
 &= \frac{(2\epsilon)^{1/p}}{1-\epsilon} n^{-(p-1)/p} = \frac{(2\epsilon)^{1/p}}{1-\epsilon} n^{-1/q}.
\end{align}
\end{proof}
\begin{corollary}
\label{cor:m-to-m-inv}
Let $W_1 = W - u \Ind^{\top}$. Then for any $m \geq 2$ and $\epsilon \leq \frac{1}{8}$, 
if $W \in \sW(\epsilon)$ then 
$\|X(I-W)(I-W_1)^{-1}\|_{2 \to m/(m-1)} \leq \frac{7}{3}\|X(I-W)\|_{2 \to m/(m-1)}$.
\end{corollary}
\begin{proof}
It suffices to bound $\|(I-W_1)^{-1}\|_{m/(m-1) \to m/(m-1)}$. But we can bound this by 
$\frac{1}{1 - \|W_1\|_{m/(m-1) \to m/(m-1)}}$. By the preceding lemma, 
$\|W_1\|_{m/(m-1) \to m/(m-1)} \leq (2\epsilon)^{(m-1)/m} / (1-\epsilon) \leq \sqrt{1/4} / (7/8) \leq \frac{4}{7}$, so the overall bound is $\frac{7}{3}$ as claimed.
\end{proof}


==> content/sum-of-squares.tex <==

%!TEX root=../main.tex

% \documentclass[11pt]{article}

% \usepackage{fullpage}
% \usepackage{times}
% \usepackage{hyperref}       % hyperlinks
% \usepackage{subcaption}
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{amsmath,amsfonts,amssymb,amsthm}
% \usepackage{graphicx}
% \usepackage{ifthen}
% \usepackage{color}

%\input latex-defs
%\usepackage{natbib}
% \definecolor{mydarkblue}{rgb}{0,0.08,0.45}                                         
% \hypersetup{
%   colorlinks=true,
%   linkcolor=mydarkblue,
%   citecolor=mydarkblue,
%   filecolor=mydarkblue,
%   urlcolor=mydarkblue,
% }
% \setcitestyle{authoryear,round,citesep={;},aysep={,},yysep={;}}
% \usepackage{tikz}
% \usetikzlibrary{patterns,positioning,fit,calc}
% \usepackage{paralist}
% \usepackage{enumitem}
% \usepackage{mathtools}
% \usepackage{algorithm,algorithmicx,algcompatible,algpseudocode}
% \usepackage{bbm}

% \newcommand{\theTitle}{Sum-of-Squares Bounds for Clustering}
% \title{\theTitle}

% \begin{document}

% \maketitle



\section{Problem Setting}
We suppose that there are points $x_1, \ldots, x_n$ that are partitioned into $k$ sets $S_1, \ldots, S_k$. 
For each set $S_j$ there is a corresponding mean $\mu_j$; we define the $4$th moment $\sigma_j$ of the set $S_j$ 
as $\sigma_j \eqdef \sigma(S_j, \mu_j)$, and let $\sigma = \max_j \sigma_j$. 
We also let $r = \max_j \|\mu_j\|_2$, and $\alpha = \min_j \alpha_j$, where $\alpha_j = |S_j|/n$. 


\section{Optimization}
We will analyze the following optimization problem:
\begin{align}
\label{eq:optimization}
\text{minimize} & \phantom{++} \sum_{i=1}^n \|w_i - x_i\|_2^2 \\
\text{subject to} & \phantom{++} w_i^{\otimes 4} \preceq Y \text{ for } i = 1,\ldots, n\\
                  & \phantom{++} \|Y\|_* \leq kr^4 \\
                  & \phantom{++} \|w_i\|_2 \leq r,
\end{align}
We remark that this is a sum-of-squares program and hence can be solved in polynomial time.

\section{Error Bound}
We claim that the following error bound holds for the result of 
\eqref{eq:optimization}:
\begin{theorem}
On average, the squared distance of points $\hat{w}_i$ to their corresponding 
cluster center is $\oo\p{k^{1/4}\sigma r}$.
\end{theorem}

\begin{proof}
Letting $\hat{w}_{1:n}$, $\hat{Y}$ be the optimal parameters for 
\eqref{eq:optimization}, we will bound the suboptimality of $\hat{w}_{1:n}$ for 
the ``true'' objective $\sum_{i=1}^n \|w_i - \mu_{j(i)}\|_2^2$ (where $j(i)$ is 
used to denote the cluster that $x_i$ belongs to).

First, since a feasible solution is to set $w_i = \mu_{j(i)}$, $Y = \sum_{j=1}^k \mu_j^{\otimes 4}$, 
by the optimality of $\hat{w}$ we have
\begin{align}
\label{eq:obj-bound}
\sum_{i=1}^n \|\hat{w}_i - x_i\|_2^2 &\leq \sum_{i=1}^n \|\mu_{j(i)} - x_i\|_2^2.
\end{align}
Next, note that
\begin{align}
\sum_{i=1}^n \|\hat{w}_i - \mu_{j(i)}\|_2^2 &= \sum_{i=1}^n \|\hat{w}_i - x_i\|_2^2 - \|\mu_{j(i)} - x_i\|_2^2 + 2\langle \hat{w}_i - \mu_{j(i)}, x_i - \mu_{j(i)} \rangle \\
 &\stackrel{\eqref{eq:obj-bound}}{\leq} 2\sum_{i=1}^n \langle \hat{w}_i - \mu_{j(i)}, x_i - \mu_{j(i)} \rangle \\
 &\stackrel{(i)}{\leq} 2n \p{\frac{1}{n} \sum_{i=1}^n \langle \hat{w}_i^{\otimes 4}, (x_i - \mu_{j(i)})^{\otimes 4} \rangle + \langle \mu_{j(i)}^{\otimes 4}, (x_i - \mu_{j(i)})^{\otimes 4} \rangle}^{1/4} \\
 &\stackrel{(ii)}{\leq} 2n \p{\frac{1}{n} \sum_{j=1}^k \sum_{i \in S_j} \big(\langle \hat{Y}, (x_i - \mu_j)^{\otimes 4} \rangle + \langle \mu_j^{\otimes 4}, (x_i - \mu)^{\otimes 4} \rangle\big)}^{1/4} \\
 &\stackrel{(iii)}{\leq} 2n \p{\frac{1}{n} \sum_{j=1}^k |S_j|(k+1)r^4\sigma^4}^{1/4} \\
\label{eq:main-bound} &\leq 2n \sigma r \p{k+1}^{1/4}.
\end{align}
Here (i) is the power mean inequality, and (ii) is re-grouping of the terms together with the fact that $\hat{w}_i^{\otimes 4} \preceq \hat{Y}$. 
Finally, (iii) makes use of the bounds $\|\hat{Y}\|_* \leq kr^4$ and $\|\mu_j^{\otimes 4}\|_* \leq r^4$, and the definition of $\sigma$.

Examining \eqref{eq:main-bound}, we obtain
\begin{align}
\frac{1}{n} \sum_{i=1}^n \|\hat{w}_i - \mu_{j(i)}\|_2^2 
  &\leq \oo\p{k^{1/4}\sigma r}.
\end{align}
\end{proof}
This shows that the $\hat{w}_i$ have averaged squared $\ell_2$ distance 
of $\oo\p{k^{1/4}\sigma r}$ to their cluster center. Whenever $k^{1/4}\sigma r \ll r^2$, 
we can cluster and re-center to get an equivalent problem where $r$ is substantially smaller. 
Therefore, we can suppose that $r \approx k^{1/4} \sigma$, hence the average squared 
$\ell_2$ distance can be made to be $k^{1/2} \sigma^2$, and we end up being able to cluster 
points to (non-squared) $\ell_2$ error $\oo \p{k^{1/4}\sigma}$. [A technical note: the re-clustering 
can actually introduce some log factors, I believe, but we'll ignore this for now.]

%{\small
%\bibliographystyle{plainnat}
%\bibliography{refdb/all}
%}
%
%\newpage
%\onecolumn
%\appendix

% \end{document}


==> refdb/.git/objects/45/c0952ec9c6e12ce69375d28b5b424da1a39c29 <==
x¥Î=!†akN1Ðÿcmë	Fã.†eïïÚxÛ§x¿/µiª"ÃÝèÌà
*M䌷T˜£e+µ7AÆàÞ
jY"oê<ˆ^Y'D2³G49²É>[œV&Jã%*T´ŽGëp¡Ônp\çõ<àøüÊaùÉù>Q}R›N -F¯ö¸õŦÛÝÁ‡Ä©Í¶­:/ëk@­âæ¦S

==> refdb/.git/objects/b8/186559bf2df3e75d6dcbd01c2f017ed6fdd659 <==
x+)JMU016e040031QÐKÏ,ÉLÏË/JeP¿^–TÈ¿¾>ï	wtÔG7·r¨*ßÄìԴ̜TÁÇ9ϼ^‡$T}põ‡Û"ê{çgæCÕ¹:ºøºêå¦0ìºûMæÅ©­Ÿšg«›õý¸uÅè»2TQbNŽ^RfCÕ姏"N.֚toݤ#J\ÝSÚ-L€@!%±$'áÚDÖsË•#Þèð,Ó[h¹í#ԄôԼԢĽ¢$†s^Å|Þô;>ç~vLd¡Îbù¼"@U榦
U%© e7¹ŸLø»àž=»ùçUÎ1Âvç: Ê2sò‹J@ŠæíÝ6m¹ÆɸI͖=r–_k§W·AmÌMÌÌÓK..fHYj4mYgaù¦«*ŸYL®t¸>›
5(73½(±$Uè7iÂ:N‡¢KC´'(ì2w]aæ¼ôó.¨iE©i)`5_ž<zµiöꋲ6h®=în+üã$ÊS"z$²,MO¼×üÿ÷œÍ¥z…ÅåK÷U³
